A Java Data Security Framework (JDSF) and its Case Studies

We present the design of something we call Confidentiality, Integrity and Authentication Sub-Frameworks, which are a part of a more general Java Data Security Framework (JDSF) designed to support various aspects related to data security (confidentiality, origin authentication, integrity, and SQL randomization). The JDSF was originally designed in 2007 for use in the two use-cases, MARF and HSQLDB, to allow a plug-in-like implementation of and verification of various security aspects and their generalization. The JDSF project explores secure data storage related issues from the point of view of data security in the two projects. A variety of common security aspects and tasks were considered in order to extract a spectrum of possible parameters these aspects require for the design an extensible frameworked API and its implementation. A particular challenge being tackled is an aggregation of diverse approaches and algorithms into a common set of Java APIs to cover all or at least most common aspects, and, at the same time keeping the framework as simple as possible. As a part of the framework, we provide the mentioned sub-frameworks' APIs to allow for the common algorithm implementations of the confidentiality, integrity, and authentication aspects for MARF's and HSQLDB's database(s). At the same time we perform a detailed overview of the related work and literature on data and database security that we considered as a possible input to design the JDSF.

==> Makefile <==
# MARF LaTeX Documentation
# Use with GNU make
#
# Serguei Mokhov
#
# Copyright (c) 2002 - 2007 The MARF Research and Development Group
#
# $Header: /cvsroot/marf/marf/doc/src/tex/inse691A/Attic/Makefile,v 1.1.2.8 2011/01/11 18:04:14 mokhov Exp $

#
# Settings
#

#PDFLATEXFLAGS = --interaction=batchmode --file-line-error-style
PDFLATEXFLAGS = --interaction=batchmode

APPDIR = ../../../../apps/SpeakerIdentApp
APPFILES = SpeakerIdentApp.tex SpeakersIdentDb.tex testing-sh.tex

ARCHDIR = ../../graphics/arch
ARCHIMAGES := \
	arch-general.png \
	classification.png \
	feature-extraction.png \
	gui.png \
	packages.png \
	pipeline-flow.png \
	pipeline.png \
	preprocessing.png \
	storage.png

DATASECDIR = ../../graphics/security/data
DATASECIMAGES := \
	encrypted-search-scheme.png \
	auth-decr-data-read.png \
	cbc-crypt.png \
	cbc-decrypt.png \
	enc-auth-data-store.png \
	hash-function.png \
	hmac-auth-process.png \
	database-security-classes.png \
	marf-dbsec-pkgs.png \
	marf-security-adapters.png \
	marf-security-algorithms.png \
	marf-security-authentication.png \
	marf-security-confidentiality.png \
	marf-security-integrity.png \
	marf-security-storage.png \
	marf-security.png \
	marf-security-integrity-watermarkdetection.png \
	marf-security-integrity-watermarkinsertion.png \
    marf-security-integrity-audiofrequencymasking.png \
    marf-security-integrity-integritylock.png \
    marf-security-authentication-staticcase.png \
    marf-security-authentication-dynamiccase.png \
    marf-security-authentication-dynamiccase-verification.png \
	sql-randomization-proxy.png \
	localized-key.png

IMGFILES := \
	$(DATASECDIR/DATASECIMAGES:%=%.png) \
	$(ARCHDIR/ARCHIMAGES:%=%.png) \


#
# Build
#

all: report

report: date.tex support-files images
	@echo "Compiling *.tex files..."
	pdflatex $(PDFLATEXFLAGS) report
	@echo "Compiling bibliography..."
	bibtex report
	@echo "Making index..."
	makeindex report
	@echo "Updating cross-references..."
	pdflatex $(PDFLATEXFLAGS) report
	pdflatex $(PDFLATEXFLAGS) report

date.tex: \
        report.tex \
        styles.tex \
        intro \
        methodology \
        references.tex
	@echo "Time-stamping..."
	date > date.tex

intro: toc.tex introduction.tex

methodology: methodology.tex

appendix: appendix.tex cvs.tex app todo

support-files: toc.tex references.tex report.bib

toc.tex: ../toc.tex
	@echo "NOTICE: Ignoring list of tables..."
	cat ../toc.tex | grep -v listoftables > toc.tex
#	ln -sf ../toc.tex

references.tex: ../references.tex
	ln -sf ../references.tex

styles.tex: ../../styles/styles.tex
	ln -sf ../../styles/styles.tex

report.bib: ../report.bib
	ln -sf ../report.bib

#
# Support Files
#

images: $(DATASECIMAGES) #$(ARCHIMAGES)

$(DATASECIMAGES):
	ln -sf $(DATASECDIR)/$@ $@

$(ARCHIMAGES):
	ln -sf $(ARCHDIR)/$@ $@


todo: TODO.tex

TODO.tex: ../../../TODO
	@echo "Preparing TODO list for insertion..."
	@echo "\begin{verbatim}" > TODO.tex
	@cat ../../../TODO | perl -e "while(<STDIN>){s/\t/    /g; print}" >> TODO.tex
	@echo "\end{verbatim}" >> TODO.tex


#
# Clean up
#

clean:
	rm -f *.log *.pdf

maintainer-clean: clean
	rm -f *.diff \
	TODO.tex date.tex \
	*.dvi *.aux *.toc *.lot *.lof *.idx *.ind *.ilg *.bbl *.blg *~

# EOF

